Differentially Private Policy Gradient

Motivated by the increasing deployment of reinforcement learning in the real world, involving a large consumption of personal data, we introduce a differentially private (DP) policy gradient algorithm. We show that, in this setting, the introduction of Differential Privacy can be reduced to the computation of appropriate trust regions, thus avoiding the sacrifice of theoretical properties of the DP-less methods. Therefore, we show that it is possible to find the right trade-off between privacy noise and trust-region size to obtain a performant differentially private policy gradient algorithm. We then outline its performance empirically on various benchmarks. Our results and the complexity of the tasks addressed represent a significant improvement over existing DP algorithms in online RL.

==> secs/old.tex <==
\subsection{Connecting Differential Privacy and Trust-Region Methods}

Our objective is now to propose a differentially private update mechanism for policy $\pi$. To this end, we consider a policy gradient update, and connect differential privacy techniques with trust-region policy updates.

Since we use policy gradient, our update mechanism $\pi_\theta \leftarrow \mathcal{M}(\pi_\theta, D^{\pi_\theta})$ becomes:
\[
    \theta \leftarrow \theta + \eta \cdot \hat{g}(D^{\pi_\theta}) \enspace,
\]
where $\hat{g}(D^{\pi_\theta})$ is the sample gradient estimated on on-policy data $D^{\pi_\theta}$, which we denote hereafter $\hat{g}$ for simplicity. In the following also denote $\theta_\text{old}$ the parameters of the policy at the current iteration (the one used to collect the data), such that $\pi_\theta$ is the new updated policy: $\theta = \theta_\text{old} + \eta \cdot \hat{g}$.

As described in Section~\ref{sec:desc_pg_methods}, the underlying idea behind trust-region methods such as TRPO and PPO is to constraint the (expected) KL divergence between $\pi_{\theta_\text{old}}$ and $\pi_\theta$:
\begin{equation} \label{eq:kl_trust_region}
    \mathbb{E} [\text{KL}(\pi_{\theta_{\text{old}}}, \pi_\theta)] \le \alpha\enspace ,
\end{equation}
where the expectation is taken on the states encountered when rolling policy $\pi_{\theta_\text{old}}$. The KL-divergence can be reasonably approximated at the second order using the Fisher information matrix of $\pi_{\theta_\text{old}}$, $F := F(\theta_\text{old})$:
\[
    \mathbb{E} \left[KL(\pi_{\theta_{\text{old}}}, \pi_\theta)\right] \approx (\theta - \theta_\text{old})^T F (\theta-\theta_\text{old}) := \Delta\theta^TF\Delta\theta \enspace .
\]
Based on our policy update formula, we have $\Delta\theta = \eta \hat{g}$. The trust-region constraint thus becomes:
\begin{equation}\label{eq:fisher_trust_region}
    \eta^2 \hat{g}^T F \hat{g} \le \alpha \enspace.
\end{equation}
(\ref{eq:fisher_trust_region}) directly links the policy gradient to the trust region constraint \textit{via} the FIM.

\subsubsection{DP Clipping and Trust Region} \label{sec:dp_clip_trust_region}

We can see rewrite (\ref{eq:fisher_trust_region}) as
\[
    \Vert \hat{g} \Vert_F \le \frac{\sqrt{\alpha}}{\eta} \enspace,
\]
where $\Vert v \Vert_F = \sqrt{v^T F v}$ is the Mahalanobis norm w.r.t. $F$.

Therefore, clipping the policy gradient $\hat{g}$ w.r.t. the norm $\Vert \cdot \Vert_F$ using clipping norm $S = \frac{\sqrt{\alpha}}{\eta}$ is roughly equivalent to guaranteeing that $\pi_\theta$ stays in the trust region defined by (\ref{eq:kl_trust_region}). Although the Gaussian mechanism is typically defined for the standard $L_2$-norm, we can adapt it to norms defined by a symmetric positive definite matrix like $\Vert \cdot \Vert_F$. Indeed, according to Proposition 3 from \citet{HallRW13}, if $\Vert \hat{g} \Vert_F = \Vert F^{1/2} \hat{g} \Vert_2 \le S$, then the following Gaussian mechanism is $(\epsilon, \delta)-DP$:
\begin{equation} \label{eq:gauss_fisher_mechanism}
    \tilde{g} = \hat{g} + \frac{C(\delta) \cdot S}{\epsilon} \cdot \zeta \enspace, \quad \zeta \sim \mathcal{N} \left(0, F^{-1} \right)\enspace,
\end{equation}
as long as $C(\delta) \ge \sqrt{2 \log\frac{2}{\delta}}$.

Using this \textit{Gauss-Fisher mechanism} to privatize the policy gradient updates is therefore (approximately) equivalent to performing trust-region updates with radius $\alpha$ and adding noise. We therefore argue that trust-region methods like TRPO and PPO already take care of the "clipping part" of differential privacy, so that the additional noise remains the only perturbation to policy convergence. This indicates that trust-region methods could behave better than expected under private constraint.

However, this approach has several limitations, mainly:
\begin{enumerate}
    %\item It relies on the estimation of $F$, which is not straightforward in high dimension
    %\item $F$ is typically estimated from the data, which raises privacy concerns
    \item The computation of $F^{-1}$ can be prohibitively expensive depending on the problem dimensionality; also, numerical issues may lead to poor noise scaling
    \item This approach does not integrate the noise within the trust-region. Therefore, the noise may lead the update to scale beyond the trust region, weakening the benefits of trust-region methods and leading to poor convergence.
\end{enumerate}

In the sequel, we propose another approach exploiting Equation (\ref{eq:fisher_trust_region}) while addressing these limitations.
